Versatile emulation of spiking neural networks on an accelerated neuromorphic substrate

We present first experimental results on the novel BrainScaleS-2 neuromorphic architecture based on an analog neuro-synaptic core and augmented by embedded microprocessors for complex plasticity and experiment control. The high acceleration factor of 1000 compared to biological dynamics enables the execution of computationally expensive tasks, by allowing the fast emulation of long-duration experiments or rapid iteration over many consecutive trials. The flexibility of our architecture is demonstrated in a suite of five distinct experiments, which emphasize different aspects of the BrainScaleS-2 system.

==> standaloneFigs/figStructural/schematic/schematic.tex <==
\begin{tikzpicture}[>=stealth,x=1.3cm,y=1.15cm]
	\def\columns{2}
	\def\rows{2}
	
	\pgfmathsetseed{1230}

	\def\spikecolors{{"red","blue","orange"}}

	\newcommand{\drawspiketrain}[4]{%
		\pgfmathsetseed{#1}
		\foreach \i in {0,1,...,200} {
			\pgfmathparse{int(random(0, 100)/1.0)}
			\ifnum \numexpr\pgfmathresult > \numexpr100-#2
				\draw[draw=#3] #4 ++ (\i*0.0035,0.05) -- ++(0,0.2);
			\fi
		}
	}

	% input from FPGA
	\begin{scope}
		\foreach \row in {0,1,...,\numexpr\rows-1} {
			\draw[black,thick] (-1.0,-\row) -- (-0.4,-\row);
			%\draw[black,thick,-stealth] (-2.5,-\row) -- (-0.55,-\row);
		}
	\end{scope}

	% input spike trains
	\begin{scope}
		%\draw[thick,black,rounded corners=0.4,fill=white] (-3.1,-1.05) rectangle ++(3.2,2.1);
		\begin{scope}
			\foreach[count=\address from 0] \strength/\color in {1/red,1/green,1/blue} {
				\draw[thick] (-2.8,-1 + 0.35*\address-0.35-0.175) -- ++(1.1,0) to[out=0,in=180] (-1.3,-1) -- (-1.0,-1);
				\pgfmathparse{\spikecolors[\address]}
				\colorlet{sc}{\pgfmathresult!100}
				\drawspiketrain{\address+1}{\strength}{sc}{(-2.8,-1 + \address*0.35-0.35-0.175)}

				\draw[draw=sc,fill=white,rounded corners=0.2] (-1.5-0.25-0.25,-1+\address*0.35-0.35+0.05-0.175) rectangle ++(0.2,0.2)
					node[pos=0.5,sc] {\texttt\address};
			}
		\end{scope}
		
		\foreach[count=\address from 0] \strength/\color in {1/red,1/green,1/blue} {
			\pgfmathparse{\spikecolors[\address]}
			\colorlet{sc}{\pgfmathresult!100}
			\drawspiketrain{\address+1}{\strength}{sc}{(-1.2,-1)}
		}
	\end{scope}

	\pgfmathsetseed{1236}
	\begin{scope}
		% synapse array
		\foreach \x in {0,1,...,\numexpr\columns-1}
			\draw[thick,black,-stealth] (\x,0.5) -- ++(0,-\rows) -- ++(0.0,-0.35);
		\foreach \y in {0,1,...,\numexpr\rows-1}
			\draw[thick,black] (-0.5,-\y) -- ++(\columns,0);

		\foreach \column in {0,1,...,\numexpr\columns-1} {
			\foreach \row in {0,1,...,\numexpr\rows-1} {
				\pgfmathparse{int(random(0,2))}
				\edef\address{\pgfmathresult}
				\pgfmathparse{\spikecolors[\address]}
				\colorlet{sc}{\pgfmathresult!100}
				
				\ifthenelse{\column = 0 \AND \row = 0} {
					\def\drawlevel{100}
					\def\filllevel{20}
					\def\textlevel{100}
				} {
					\def\drawlevel{20}
					\def\filllevel{5}
					\def\textlevel{50}
				}
				\draw[draw=black!\drawlevel,fill=white,rounded corners=1.0] (\column,\row-1) ++ (-0.2,0.15) rectangle ++(0.4,-0.6);
				\draw[draw=black!\drawlevel] (\column,\row-1) ++ (-0.2,-0.15) -- ++(0.4,0);
				\draw[draw=none] (\column,\row-1) ++ (-0.2,0.15) rectangle ++(0.4,-0.3) node[pos=0.5,color=sc!\textlevel] {\texttt\address};
				\draw[draw=none] (\column,\row-1) ++ (0,-0.45) ++ (-0.2,-0.0) rectangle ++(0.4,0.3)
					node[pos=0.5,color=black!\textlevel] {\pgfmathparse{int(random(0,63))}\texttt\pgfmathresult};

				% correlation sensors
				%\draw[draw=orange!\drawlevel,fill=orange!\filllevel,rounded corners=0.2] (\column,-\row) ++ (0,-0.38) ++ (0.28,-0.15) rectangle ++(0.1,0.68);
				%\draw[draw=orange!\drawlevel,fill=orange!\drawlevel,rounded corners=0.2] (\column,-\row) ++ (0,-0.38) ++ (0.28,-0.15) rectangle ++(0.1,{((rand+1)/2)*0.68});
			}
		}
	\end{scope}

	% neurons
	\begin{scope}
		\foreach \neuron in {0,...,\numexpr\columns-1} {
			\ifthenelse{\neuron = 0} {
				\def\drawlevel{100}
				\def\filllevel{20}
				\def\textlevel{100}
			} {
				\def\drawlevel{20}
				\def\filllevel{5}
				\def\textlevel{50}
			}
			
			\draw (\neuron,-\rows-0.4) ++(0.3,-0.1) -- ++(-0.3,0.55) -- ++(-0.3,-0.55) -- cycle;
			\draw (\neuron,-\rows-0.3) node[] {\neuron};

			% rate counter
			%\draw[draw=purple!\drawlevel,fill=purple!\filllevel] (\neuron,-\rows) ++ (-0.3,-1.6) rectangle ++(0.6,-0.4)
			%	node[pos=0.5,color=purple!\textlevel] {\pgfmathparse{int(random(0,255))}\pgfmathresult};
		}
	\end{scope}	

	% PPU
	%\begin{scope}
	%	\foreach \col in {0,1,...,\numexpr\columns-1} {
	%		\ifthenelse{\col = 0} {
	%			\def\drawlevel{100}
	%		} {
	%			\def\drawlevel{20}
	%		}
	%		%\draw[thick,blue!\drawlevel,stealth-] 		(\col-0.4,1) -- ++(0,-\rows-2.6) -- ++(0.08,0);
	%		%\draw[thick,blue!\drawlevel,stealth-stealth] 	(\col-0.4,1) -- (\col-0.4,0.1) -- ++(0.17,0);
	%		%\draw[thick,blue!\drawlevel,stealth-stealth] 	(\col-0.4,1) -- (\col-0.4,-0.28) -- ++(0.17,0);
	%		%\draw[thick,blue!\drawlevel,stealth-] 		(\col+0.33,1) -- ++(0,-0.850);
	%	}

	%	\draw[thick,blue] (-0.5,1) rectangle ++(\columns,0.8) node[pos=0.5] {PPU};
	%\end{scope}
\end{tikzpicture}

